Stability properties of gradient flow dynamics for the symmetric low-rank matrix factorization problem

The symmetric low-rank matrix factorization serves as a building block in many learning tasks, including matrix recovery and training of neural networks. However, despite a flurry of recent research, the dynamics of its training via non-convex factorized gradient-descent-type methods is not fully understood especially in the over-parameterized regime where the fitted rank is higher than the true rank of the target matrix. To overcome this challenge, we characterize equilibrium points of the gradient flow dynamics and examine their local and global stability properties. To facilitate a precise global analysis, we introduce a nonlinear change of variables that brings the dynamics into a cascade connection of three subsystems whose structure is simpler than the structure of the original system. We demonstrate that the Schur complement to a principal eigenspace of the target matrix is governed by an autonomous system that is decoupled from the rest of the dynamics. In the over-parameterized regime, we show that this Schur complement vanishes at an $O(1/t)$ rate, thereby capturing the slow dynamics that arises from excess parameters. We utilize a Lyapunov-based approach to establish exponential convergence of the other two subsystems. By decoupling the fast and slow parts of the dynamics, we offer new insight into the shape of the trajectories associated with local search algorithms and provide a complete characterization of the equilibrium points and their global stability properties. Such an analysis via nonlinear control techniques may prove useful in several related over-parameterized problems.

==> commandsHesam.tex <==
% =============================================================================
% Hesameddin Mohammdi
% The basic set of user-defined commands
% =============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*\mystrut[1]{\vrule width0pt height0pt depth#1\relax}
\DeclareMathOperator{\EX}{\mathbb{E}}
\newcommand{\hmmargin}[1]{\marginnote{\color{blue!80!white}\tiny\ttfamily{HM:} #1}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\DefinedAs}[0]{\mathrel{\mathop:}=}
\newcommand{\AsDefined}[0]{=\mathrel{\mathop:}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\logdet}{log\,det}
\DeclareMathOperator*{\vecform}{vec}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\subject}{subject~to}
\DeclareMathOperator*{\rank}{rank}

\newcommand{\new}{{\rm new}}
\newcommand{\old}{{\rm old}}
\newcommand{\barp}{{\bar p}}
\newcommand{\Diag}{{\rm Diag}\;}
\newcommand{\CP}{{\cal P}}
\newcommand{\rmCAP}{{\rm CAP}}
\newcommand{\epc}{\hspace{1pc}}
\newcommand{\gap}{\vspace{0.1in}}
\newcommand{\Mbld}{{\mbox{\bf M}}}
\newcommand{\Xbld}{{\mbox{\bf X}}}
\newcommand{\qbld}{{\mbox{\bf q}}}
\newcommand{\scmax}{{\rm {\scriptstyle max}}}
\newcommand{\sign}{{\rm {\scriptstyle sign}}}
\newcommand{\scdia}{{\rm {\scriptstyle dia}}}
\newcommand{\sclow}{{\rm {\scriptstyle low}}}
\newcommand{\scupp}{{\rm {\scriptstyle upp}}}

\newcommand{\abs}[1]{\lvert #1 \rvert} 




\newcommand{\tc}{\textcolor}
\newcommand{\vsp}{\vspace*{0.15cm}}
\newcommand{\atan}{\mathrm{atan}}

\newtheorem{mydef}{Definition}
\newtheorem{mythm}{Theorem}
\newtheorem{myprop}{Proposition}
\newtheorem{mylem}{Lemma}
\newtheorem{myrem}{Remark}
\newtheorem{myass}{Assumption}
\newtheorem{myfp}{Feasibility Problem}
\newtheorem{mycor}{Corollary}

\newcommand{\one}{\mathds{1}}
\newcommand{\qedsymbol}{$\blacksquare$}
\DeclareMathOperator*{\Null}{Null}

\newcommand{\Lf}{L}
\newcommand{\mf}{m}







